CEL: Comprehensive Counterfactual Explanations Library and Benchmark

Counterfactual explanations are a prominent approach in explainable artificial intelligence (xAI), providing actionable guidance on what input changes would alter a model's prediction to a desired outcome. While early methods primarily focused on minimal feature changes, recent work incorporates additional properties such as sparsity, actionability and plausibility. Despite this progress, fair and systematic evaluation remains challenging. Existing studies often rely on different data splits, predictive models, and evaluation metrics, which limits objective comparison across methods. To fill this gap, we introduce CEL (Counterfactual Explanations Library), a unified library and benchmark for counterfactual explanations designed to support consistent implementation and evaluation. CEL includes 18 datasets of varying size and complexity and provides implementations or reimplementations of 14 widely used counterfactual methods. Using this standardized setup, we conduct a comprehensive quantitative comparison across a variety of methods on datasets that differ in size, number, and types of attributes. The evaluation protocol incorporates multiple complementary metrics capturing validity, coverage, sparsity, proximity, and distributional plausibility, including density- and outlier-based measures to assess the realism of generated counterfactuals. To the best of our knowledge, this is the first comprehensive benchmark that systematically evaluates recent counterfactual explanation methods within a unified and reproducible framework. While prior libraries and benchmarking efforts exist in the literature, many are outdated, limited in scope, or lack consistent evaluation protocols. The proposed benchmark aims to improve reproducibility, enable fair comparison, and establish a workbench for the development of future counterfactual explanation methods.

==> small-tables/results_adult_census_group.tex <==
\begin{table}[h]
\centering
\caption{Metrics for a single dataset.}
\label{tab:group_adult_census}
\begin{center}
\begin{sc}
\begin{scriptsize}
\begin{tabular}{l|rrr}
\toprule
Method & Valid.$\uparrow$ & L2-Jac.$\downarrow$ & Log Dens.$\uparrow$ \\
\midrule
TCREx & $0.23\pm{0.02}$ & $\boldsymbol{0.00\pm{0.00}}$ & $\boldsymbol{-242.83\pm{13.92}}$ \\
GroupGLANCE & $\boldsymbol{0.99\pm{0.01}}$ & $0.80\pm{0.03}$ & $-251.57\pm{80.02}$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{sc}
\end{center}
\end{table}


==> small-tables/results_gmsc_global.tex <==
\begin{table}[h]
\centering
\caption{Metrics for a single dataset.}
\label{tab:global_give_me_some_credit}
\begin{center}
\begin{sc}
\begin{scriptsize}
\begin{tabular}{l|rrr}
\toprule
Method & Valid.$\uparrow$ & Euc.-Jac.$\downarrow$ & Log Dens.$\uparrow$ \\
\midrule
AReS & $0.88\pm{0.10}$ & $0.42\pm{0.00}$ & $\boldsymbol{-14.81\pm{5.71}}$ \\
GLOBE-CE & $\boldsymbol{1.00\pm{0.00}}$ & $\boldsymbol{0.01\pm{0.01}}$ & $-15.17\pm{6.03}$ \\
GlobalGLANCE & $\boldsymbol{1.00\pm{0.00}}$ & $0.79\pm{0.00}$ & $-27.54\pm{10.15}$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{sc}
\end{center}
\end{table}


==> small-tables/results_law_local.tex <==
\begin{table}[h]
\centering
\caption{Results for logistic regression on Law dataset. Presented results show strenghts of different explanation methoods. CCHVAE and PPCEF target plausibility which makes them achieve better logarithmic density than their counterparts. Gradient based optimization used for PPCEF allows to easily combine logarithmic density with better proximity metrics. }
\label{tab:results_law_local}
\begin{center}
\begin{sc}
\begin{scriptsize}
\begin{tabular}{l|rrr}
\toprule
Method & Valid.$\uparrow$ & L2-Jac.$\downarrow$ & Log Dens.$\uparrow$ \\
\midrule
CADEX & $\boldsymbol{1.00\pm{0.00}}$ & $0.18\pm{0.03}$ & $-12.77\pm{0.97}$ \\
CCHVAE & $\boldsymbol{1.00\pm{0.00}}$ & $0.11\pm{0.01}$ & $\boldsymbol{-10.52\pm{0.95}}$ \\
SACE & $\boldsymbol{1.00\pm{0.00}}$ & $0.45\pm{0.19}$ & $-13.74\pm{2.11}$ \\
DiCE & $0.92\pm{0.04}$ & $0.24\pm{0.00}$ & $-17.70\pm{1.05}$ \\
PPCEF & $\boldsymbol{1.00\pm{0.00}}$ & $\boldsymbol{0.06\pm{0.01}}$ & $-11.31\pm{1.06}$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{sc}
\end{center}
\end{table}


==> small-tables/results_regression_representative.tex <==
\begin{table}[h]
\centering
\caption{Comparative regression results for the \textbf{Linear Regression} model. Main performance metrics.}
\label{tab:regression_lr_representative}
\begin{center}
\begin{sc}
\begin{tiny}
\begin{tabular}{ @{}llrrr @{}}
\toprule
Dataset & Method & MAE $\downarrow$ & L2 $\downarrow$ & Log Dens. $\uparrow$ \\
\midrule
\multirow[t]{3}{*}{Synthetic} & CEARM & 0.05$\pm$0.01 & 0.38$\pm$0.03 & -83.59$\pm$52.05 \\
 & WACH & 0.06$\pm$0.01 & \textbf{0.15$\pm$0.02} & 0.87$\pm$2.27 \\
\midrule
\multirow[t]{3}{*}{Concrete} & CEARM & 0.03$\pm$0.00 & 1.13$\pm$0.02 & -2880.93$\pm$3261.61 \\
 & WACH & 0.05$\pm$0.00 & \textbf{0.16$\pm$0.00} & 0.45$\pm$2.17 \\
\bottomrule
\end{tabular}
\end{tiny}
\end{sc}
\end{center}
\end{table}


==> small-tables/results_wine_local.tex <==
\begin{table}[h]
\centering
\caption{Performance of local counterfactual explanation methods on the Wine dataset. We report validity (proportion of counterfactuals achieving the desired prediction, higher is better), L2--Jaccard distance as a proximity measure (lower is better), and log-density as an estimate of plausibility under the data distribution (higher is better). Results are shown as mean $\pm$ standard deviation across evaluation runs. Best values per metric are highlighted in bold.}
\label{tab:results_wine_local}
\begin{center}
\begin{sc}
\begin{scriptsize}
\begin{tabular}{l|rrr}
\toprule
Method & Valid.$\uparrow$ & L2-Jac.$\downarrow$ & Log Dens.$\uparrow$ \\
\midrule
Artelt & $\boldsymbol{1.00\pm{0.00}}$ & $0.59\pm{0.09}$ & $-19.22\pm{19.19}$ \\
CADEX & $\boldsymbol{1.00\pm{0.00}}$ & $\boldsymbol{0.37\pm{0.02}}$ & $-3.39\pm{2.18}$ \\
CCHVAE & $\boldsymbol{1.00\pm{0.00}}$ & $0.86\pm{0.04}$ & $2.96\pm{2.98}$ \\
CEGP & $\boldsymbol{1.00\pm{0.00}}$ & $\boldsymbol{0.37\pm{0.05}}$ & $-2.34\pm{1.42}$ \\
CEM & $\boldsymbol{1.00\pm{0.00}}$ & $0.63\pm{0.10}$ & $-26.30\pm{9.67}$ \\
SACE & $\boldsymbol{1.00\pm{0.00}}$ & $1.30\pm{0.11}$ & $1.74\pm{2.11}$ \\
DiCE & $0.94\pm{0.09}$ & $0.95\pm{0.05}$ & $-36.04\pm{28.43}$ \\
PPCEF & $\boldsymbol{1.00\pm{0.00}}$ & $0.52\pm{0.07}$ & $\boldsymbol{5.78\pm{1.13}}$ \\
WACH & $\boldsymbol{1.00\pm{0.00}}$ & $0.42\pm{0.05}$ & $-3.74\pm{3.13}$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{sc}
\end{center}
\end{table}

